ViLA: Efficient Video-Language Alignment for Video Question Answering

In this work, we propose an efficient Video-Language Alignment (ViLA) network. Our ViLA model addresses both efficient frame sampling and effective cross-modal alignment in a unified way. In our ViLA network, we design a new learnable text-guided Frame-Prompter together with a new cross-modal distillation (QFormer-Distiller) module. Pre-trained large image-language models have shown promising results on problems such as visual question answering (VQA). However, how to efficiently and effectively sample video frames when adapting pre-trained large image-language model to video-language alignment is still the major challenge. Compared with prior work, our ViLA model demonstrates the capability of selecting key frames with critical contents, thus improving the video-language alignment accuracy while reducing the inference latency +3.3% on NExT-QA Temporal with 3.0X speed up). Overall, our ViLA network outperforms the state-of-the-art methods on the video question-answering benchmarks: +4.6% on STAR Interaction, +2.2% on STAR average with 3.0X speed up, ours 2-frames out-perform SeViLA 4-frames on the VLEP dataset with 4.2X speed-up. The code will be available at https://github.com/xijun-cs/ViLA.

==> 13_ljb.tex <==
\clearpage
%0.011 0.256 0.5 ; 0.135 0.547 0.56 0.976
\newcommand\boxa[1]{\adjustbox{trim={.011\width} {.453\height} {.5\width} {.135\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
% \newcommand\boxb[1]{\adjustbox{trim={.256\width} {.453\height} {.5\width} {.135\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
\newcommand\boxc[1]{\adjustbox{trim={.5\width} {.453\height} {.011\width} {.135\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
% \newcommand\boxd[1]{\adjustbox{trim={.744\width} {.453\height} {.011\width} {.135\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
\newcommand\boxe[1]{\adjustbox{trim={.011\width} {.024\height} {.5\width} {.56\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
% \newcommand\boxf[1]{\adjustbox{trim={.256\width} {.024\height} {.5\width} {.56\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
\newcommand\boxg[1]{\adjustbox{trim={.5\width} {.024\height} {.011\width} {.56\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
% \newcommand\boxh[1]{\adjustbox{trim={.744\width} {.024\height} {.011\width} {.56\height},clip}{\includegraphics[height=0.5\linewidth]{#1}}}
\newcommand\showrow[1]{\multirow{2}{*}{\begin{tabular}{cc}Selected\\ frames\end{tabular}}&\boxa{#1}&\boxe{#1}\vspace{-.45em}\\&\boxc{#1}&\boxg{#1}}
\begin{table*}[!ht]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        & Ours & SeViLA \\
        
        \midrule
        Question & \multicolumn{2}{c}{How does the man sweep the pile of leaves away?} \\
        \midrule
        \showrow{figs/visualization_candidates/CH_3046900922_8.jpg} \\
        \midrule
        Answer & Swinging the boy & With a shovel \\
        \midrule
        
        \midrule
        Question & \multicolumn{2}{c}{How does one of the dog keep the other one pinned to the ground in the middle?} \\
        \midrule
        \showrow{figs/visualization_candidates/CH_3345608051_7.jpg} \\
        \midrule
        Answer & Bite its neck & Push it \\
        \midrule
        
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> constants.tex <==
\def\cvprPaperID{12999}
\def\confName{CVPR}
\def\confYear{2024}

%\def\paperTitle{BLVQA: Bootstrapping Language-Video Molding for Video Question Answering}

\def\paperTitle{VLA: Efficient Video-Language Alignment for Video Question Answering}

% BELA: Bootstrapping Efficient Language-Video Alignment for Video Question Answering


\def\authorBlock{
    Xijun Wang$^{1,2}$,
    Junbang Liang$^{2}$,
    Chun-Kai Wang$^{2}$, Kenan Deng$^{2}$, Yu Lou$^{2}$,  Ming Lin$^{1,2}$, Shan Yang$^{2}$\\
    $^1$University of Maryland, College Park \qquad $^2$Amazon \\
    {\small \{xijun, lin\}@umd.edu, \{junbangl, kenanden, ckwang, ylou, ssyang\}@amazon.com}
}


% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}



==> tables/frame_acc.tex <==
\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\# Frame & NExT-QA & STAR & How2QA & VLEP & TVQA  \\
\midrule
ViLA (1)   &    70.5 & 56.0 & 80.0   &  68.1 & 56.2 \\
ViLA (2)   &    72.8 & 62.9 & 82.8   &  69.3 &  60.6\\
ViLA (4)   &    74.4 & 67.1 & 83.9   &  69.6 &  63.4\\
ViLA (8)   &    74.8 & 67.9 & 84.5   &  69.5 &  64.0 \\
\bottomrule 
\end{tabular}
}
\caption{{\bf ViLA Results in terms of different frame number.} ViLA's performance gets better, as the number of frames increases due efficient frame setting. }
\label{tab:frame_acc}
\end{table}

% ViLA (4)   &    70.1 & 73.8 & 82.1   &  74.4 &  \\
% ViLA (8)   &    71.4 & 73.6 &  81.4   &  74.8 &  \\
% %ViLA (16)   &   69.5 & 74.0 &  81.7   &  75.0\\
% ViLA (32)   &   72.3  & 74.9 &  82.1   &  75.5 &  \\

==> tables/hyperparameters.tex <==
\begin{table*}[!h]
\centering
\begin{tabular}{cccccc}
\toprule
Datasets  & Learning Rate & Batch Size  & Warmup Step & Gradient Accumulation Step & Epoch  \\
\midrule
\multicolumn{6}{c}{Teacher} \\
\midrule
NExT-QA & 1e-5 & 2 & 500 & 4 & 10 \\
STAR & 1e-5 & 2 & 500 & 4 & 10 \\
How2QA & 2e-5 & 4 & 1400 & 2 & 10 \\
TVQA & 1e-5 & 8 & 1000 & 2 & 10 \\
VLEP & 1e-5 & 2 & 500 & 4 & 10 \\
\midrule
\multicolumn{6}{c}{Student} \\
\midrule
NExT-QA & 1e-5 & 8 & 1000 & 2 & 10 \\
STAR & 1e-5 & 8 & 1000 & 2 & 10 \\
How2QA & 2e-5 & 4 & 1400 & 2 & 10 \\
TVQA & 1e-5 & 8 & 1000 & 2 & 10 \\
VLEP & 3e-5 & 4 & 1000 & 8 & 10 \\
\bottomrule 
\end{tabular}
\caption{{\bf ViLA training hyper-parameters.} }
\label{tab:hyperparam}
\end{table*}

==> tables/teacher_size.tex <==

\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c c c}
\toprule
Teacher's Frame number & T & C & D & Average  \\
% \midrule
% 32 frames   &   69.1 & 73.6 & 81.3  &  \textbf{74.2} \\
% 32 frames  &   - & - & -  &  \textbf{74.4}\\
% 4 frames  &   71.2 & 73.0 & 80.6  &  \textbf{73.8}\\
% 8 frames  &   - & - & -  &  \textbf{74.4}\\
% 16 frames  &   70.7 & 73.4 & 80.1  &  \textbf{73.6}\\
% 32 frames  &    70.1 & 73.75 & 82.1  &  \textbf{74.4}\\

\midrule
4 frames  &   71.2 & 73.0 & 80.6  &  73.8\\
8 frames  &   71.0 & 72.9 & 82.5  &  74.3\\
16 frames  &   70.7 & 73.4 & 80.1  &  73.6\\
32 frames  &    70.1 & 73.8 & 82.1  &  74.4\\

\bottomrule 
\end{tabular}
}
\caption{{\bf ViLA Results on NExT-QA.} Fewer frame teacher can maintain better temporal alignment. Lager frame teacher can offer better causal and detail description instruction. Temporal (T), Causal (C), Description (D) \XW{keep it here or remove it or supplementary}}
\label{tab:nextqa_teacher_size}
\end{table}

==> tables/teacher_size_new.tex <==

\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c c}
\toprule
Teacher's Frame number & NExT-QA & TVQA & STAR  \\
\midrule
4 frames  &   73.8 & 63.1 & 66.4\\
8 frames  &   74.3 & 63.4 & 67.1\\
16 frames  &  73.6 & 63.0 & 65.9\\
32 frames  &  74.4 & 62.7 & 66.5\\
\bottomrule 
\end{tabular}
}
\caption{{\bf ViLA Ablation Study on Teacher Frame Number.} On all 3 datasets, the best performance is achieved when distilling with a teacher frame number of 8.}
\label{tab:nextqa_teacher_size_new}
\vspace{-5mm}
\end{table}
